On the Complexity of Solving a Bivariate Polynomial System

We study the complexity of computing the real solutions of a bivariate polynomial system using the recently proposed algorithm BISOLVE. BISOLVE is a classical elimination method which first projects the solutions of a system onto the $x$- and $y$-axes and, then, selects the actual solutions from the so induced candidate set. However, unlike similar algorithms, BISOLVE requires no genericity assumption on the input nor it needs any change of the coordinate system. Furthermore, extensive benchmarks from \cite{bes-bisolve-2011} confirm that the algorithm outperforms state of the art approaches by a large factor. In this work, we show that, for two polynomials $f,g\in\mathbb{Z}[x,y]$ of total degree at most $n$ with integer coefficients bounded by $2^\tau$, BISOLVE computes isolating boxes for all real solutions of the system $f=g=0$ using $\Otilde(n^8\tau^{2})$ bit operations, thereby improving the previous record bound by a factor of at least $n^{2}$.

==> conclusions.tex <==

We have derived a bound on the bit complexity of the algorithm \bs to isolate the real solutions of a bivariate polynomial system. To the best of our knowledge, the derived complexity bound improves considerably upon the best known complexity bounds to date.
Still, we suppose that the derived bounds are not tight and there is room for improvement. This mainly stems from the fact that the number of solutions of a bivariate system is in most cases largely 
overestimated while, at the same time, this number is intimately bound up 
with the root separation and coefficient bitlength of the resultant. 
We find it, therefore, reasonable to invest some research in the theory of \emph{sparse resultants} where the geometry of exponent vectors of input polynomials is analyzed to obtain sharp estimates. 
A bottleneck in the current analysis
is the isolation of the resultant polynomial which is assumed to be a general polynomial
of magnitude $(n^2,n(\tau+\log n))$. Hence, the question arises whether isolating the roots of a resultant is possibly easier than of a general polynomial?
Finally, it might be possible to improve the complexity of the validation step by considering asymptotically fast algorithms for multipoint polynomial evaluation~\cite{multipoint-04}.

